Pick-and-place Manipulation Across Grippers Without Retraining: A Learning-optimization Diffusion Policy Approach

Current robotic pick-and-place policies typically require consistent gripper configurations across training and inference. This constraint imposes high retraining or fine-tuning costs, especially for imitation learning-based approaches, when adapting to new end-effectors. To mitigate this issue, we present a diffusion-based policy with a hybrid learning-optimization framework, enabling zero-shot adaptation to novel grippers without additional data collection for retraining policy. During training, the policy learns manipulation primitives from demonstrations collected using a base gripper. At inference, a diffusion-based optimization strategy dynamically enforces kinematic and safety constraints, ensuring that generated trajectories align with the physical properties of unseen grippers. This is achieved through a constrained denoising procedure that adapts trajectories to gripper-specific parameters (e.g., tool-center-point offsets, jaw widths) while preserving collision avoidance and task feasibility. We validate our method on a Franka Panda robot across six gripper configurations, including 3D-printed fingertips, flexible silicone gripper, and Robotiq 2F-85 gripper. Our approach achieves a 93.3% average task success rate across grippers (vs. 23.3-26.7% for diffusion policy baselines), supporting tool-center-point variations of 16-23.5 cm and jaw widths of 7.5-11.5 cm. The results demonstrate that constrained diffusion enables robust cross-gripper manipulation while maintaining the sample efficiency of imitation learning, eliminating the need for gripper-specific retraining. Video and code are available at https://github.com/yaoxt3/GADP.

==> table-exp-success-rate-ablation.tex <==
\begin{table}[!t]
  \begin{center}
    \caption{Ablation study.}
    \label{tab:ablation}
    \begin{tabular}{l|c|c|c|c|c|c} 
        \toprule[1.5pt]
        \midrule[0.2pt]
        \multicolumn{7}{c}{\textcolor{Salmon}{object:} {Block}}\\
        \midrule
       Method & $\mathbb{G}_0$ & $\mathbb{G}_1$ & $\mathbb{G}_2$ & $\mathbb{G}_3$ & $\mathbb{G}_4$ & $\mathbb{G}_5$ \\
      \midrule
      Ours w/o Projection & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 \\
      Ours w/o $\mathcal{G}^*_{\text{prob}}$ & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 \\
      Ours & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 \\
    %\midrule[0.2pt]
    %KL(\textcolor{red}{$\mathcal{G}^{*(i)}_{\text{prob}}$},\textcolor{red}{$\mathcal{G}^{*(1)}_{\text{prob}}$}) & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
    \midrule[0.2pt]
    
    \multicolumn{7}{c}{\textcolor{Salmon}{object:} {Banana}}\\
    \midrule
    Ours w/o Projection & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 \\
      Ours w/o $\mathcal{G}^*_{\text{prob}}$ & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 \\
      Ours & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 \\
    \midrule[0.2pt]\bottomrule[1.5pt]
    \end{tabular}
  \end{center}
  
\end{table} 
